Your MMM is Broken: Identification of Nonlinear and Time-varying Effects in Marketing Mix Models

Recent years have seen a resurgence in interest in marketing mix models (MMMs), which are aggregate-level models of marketing effectiveness. Often these models incorporate nonlinear effects, and either implicitly or explicitly assume that marketing effectiveness varies over time. In this paper, we show that nonlinear and time-varying effects are often not identifiable from standard marketing mix data: while certain data patterns may be suggestive of nonlinear effects, such patterns may also emerge under simpler models that incorporate dynamics in marketing effectiveness. This lack of identification is problematic because nonlinearities and dynamics suggest fundamentally different optimal marketing allocations. We examine this identification issue through theory and simulations, wherein we explore the exact conditions under which conflation between the two types of models is likely to occur. In doing so, we introduce a flexible Bayesian nonparametric model that allows us to both flexibly simulate and estimate different data-generating processes. We show that conflating the two types of effects is especially likely in the presence of autocorrelated marketing variables, which are common in practice, especially given the widespread use of stock variables to capture long-run effects of advertising. We illustrate these ideas through numerous empirical applications to real-world marketing mix data, showing the prevalence of the conflation issue in practice. Finally, we show how marketers can avoid this conflation, by designing experiments that strategically manipulate spending in ways that pin down model form.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> supplemental_tex/illustration_parent.tex <==
Here we provide an illustration for Remark \ref{interrelated}. We generated a ``common parent'' variable $\xi_t$ as a cosine function of time (Figure \ref{fig:commonp_xi}). Next, we generated $\beta_t$ as a GP over $\xi_t$  and $x_t$ as two invertible (log and square limited to the positive domain) and two non-invertible (square and cosine) functions of $\xi_t$. The response variable was generated under time-varying DGP:

\begin{equation*}
    y_t = a_0 + \beta_t x_t + \varepsilon_t
\end{equation*}

\begin{figure}[h]
    \centering
    \caption{Common parent: $\xi_t$ over time}
    \includegraphics[width = 0.7\textwidth]{fig/common_parent/xi.png}
    \label{fig:commonp_xi}
\end{figure}

\begin{figure}[h]
    \centering
    \caption{Common parent: $\beta_t$ is a GP over $\xi_t$}
    \includegraphics[width = 0.7\textwidth]{fig/common_parent/betaxi.png}
    \label{fig:commonp_betaxi}
\end{figure}

\begin{figure}[h]
    \centering
    \caption{Common parent: $\beta_t$ over time}
    \includegraphics[width = 0.7\textwidth]{fig/common_parent/betatime.png}
    \label{fig:commonp_betatime}
\end{figure}

We estimate a static nonlinear GP model and a linear model with time-varying GP coefficients for each of the four functional forms of $x_t$. Figure \ref{fig:commonp_res} presents the results. As stated in Remark \ref{interrelated}, for the top two rows (corresponding to invertible functions of $x_t$ over $\xi_t$), the DGP can be fully expressed as a static non-linear DGP, which is picked up by the static nonlinear Gaussian Process model and results in a lower MSE on a holdout sample compared to the time-varying GP model, representing the true underlying DGP.

\begin{figure}[htbp]
    \centering
    \caption{Common parent: Invertible vs non-invertible $x(\xi_t)$}
    \includegraphics[width = \textwidth]{fig/common_parent/funcs.png}
    \label{fig:commonp_res}
\end{figure}

In the bottom two rows, the funciton of $x_t$ over $\xi_t$ is no longer monotone, and thus $y_t$ over $x_t$ is not guaranteed to have a representation as a static nonlinear DGP. Row 3 ($x_t$ is a squared function of $\xi_t$) provides an illustration. For $x_t \ge 0.6$, $y_t$ ``splits'' into two separate functions. The time-varying GP model is able to accurately capture this pattern, while the nonlinear GP model can only predict the mean of the ``split''. As a result, the time-varying GP model has a lower MSE.

The last row, however, illustrates, that invertibility of $x_t$ as a function of $\xi_t$ is not a necessary condition for $y_t$ over $x_t$ to be adequately captured by a static nonlinear DGP. Even though $x_t$ is a nonmonotone cosine function of $x_t$, $y_t$ over $x_t$ still looks nonlinear, and the static GP model provides a lower MSE compared to the time-varying GP model.

==> supplemental_tex/sim_results_w_hill.tex <==


\begin{table}[p]
\centering
\begin{tabular}{llrrrrrrrr}
\toprule
 & & \multicolumn{2}{c}{{Nonlinear DGP}} & &\multicolumn{2}{c}{{Dynamic DGP}} & &\multicolumn{2}{c}{{Hill DGP}} \\
\cmidrule(lr){3-4} \cmidrule(l){6-7} \cmidrule(l){9-10}
                {Variable} & {Level}  & {Coef} &  {$P(>\!|t|)$}    & & {Coef} & {$P(>\!|t|)$}  & & {Coef} & {$P(>\!|t|)$} \\
\midrule
Amplitude, $f$: & Low     & - & - & & - & - & & - & - \\
 & Middle & -0.06         & 0.94        &                  & 2.94          & 0.01  &  & - & -                     \\
&   High  & -0.11         & 0.88        &                  & 8.99          & 0.00  &  & - & -                     \\
\midrule
Smoothness, $f$: & Low & - & - & & - & - & & - & - \\
 & Middle & 9.99          & 0.00       &                   & 3.44          & 0.00        & & - & -               \\
 & High   & 19.43         & 0.00       &                   & 8.10          & 0.00        & & - & -               \\
 \midrule
 Infliction point, $f$: & Low & - & - & & - & - & & - & - \\
 & Middle & -         & -       &                   & -          & -             & & -2.15 & 0.21          \\
 & High   & -         & -       &    -              & -        & -              & & 2.27 & 0.19         \\
 \midrule
 Shape parameter, $f$: & Very Low & - & - & & - & - & & - & - \\
  & Low & -          & -       &                   & -          & -         & & -2.44 & 0.27             \\
 & Middle & -          & -       &                   & -          & -         & & -7.06 & 0.00              \\
 & High   & -         & -       &                   & -          & -        & & -12.14 & 0.00              \\
  & Very High   & -         & -       &                   & -          & -       & & -15.44 & 0.00               \\
 \midrule
AR coef, $x$: & Low & - & - & & - & - & & - & - \\ 
 & Middle            & 0.81          & 0.28        &                  & 1.05          & 0.36          & & -0.10 & 0.95            \\
& High            & 2.66          & 0.00          &                & 4.77          & 0.00      & & 24.22 & 0.00                 \\
\midrule
Variance, $x$: & Low  & - & - & & - & - & & - & -\\
& Middle         & -0.16         & 0.83           &               & 5.80          & 0.00   & & - & -                    \\
& High        & 0.07          & 0.92               &           & 11.66         & 0.00    & & - & -                   \\
\midrule
Noise, $y$ & Low & - & - & & - & - & & - & - \\
& Middle       & 7.60          & 0.00             &             & 6.69          & 0.00    & & 11.16 & 0.00                  \\
& High       & 14.81         & 0.00              &            & 20.25         & 0.00    & & 20.20 & 0.00                   \\
& Very High     & 24.02         & 0.00           &               & 40.19         & 0.00    & & 27.00 & 0.00                   \\
\bottomrule
\end{tabular}
\tcaption{Simulation Results}{DV = Percentage Conflation; Intercept omitted for clarity.}
\label{tab:sim_deep_dive}
\end{table}

==> supplemental_tex/tikz_diagram_parent.tex <==

\begin{figure}
    \centering
    \begin{tikzpicture}
    % Variables
    \node[const]   (t)   {$t$}; %
    \node[const, below=of t, xshift=-0.8cm]   (x)   {$x_t$}; %
    \node[const, below=of t, xshift=0.8cm]   (beta)   {$\beta_t$}; %

    % Edges
    \edge {t} {x};
    \edge {t} {beta};
    
    \end{tikzpicture}
    \hfill
    \begin{tikzpicture}
    % Variables
    \node[const]   (t)   {$t$}; %
    \node[const, below=of t, xshift=-0.8cm]   (x)   {$x_t$}; %
    \node[const, below=of t, xshift=0.8cm]   (beta)   {$\beta_t$}; %

    % Edges
    \edge {t} {x};
    \edge {t} {beta};
    \draw[->,blue] (x) to[out=45,in=135] (beta);
    
    \end{tikzpicture}
    \hfill
    \begin{tikzpicture}
    % Variables
    \node[const]   (t)   {$t$}; %
    \node[const, below=of t, xshift=-0.8cm]   (x)   {$x_t$}; %
    \node[const, below=of t, xshift=0.8cm]   (beta)   {$\beta_t$}; %

    % Edges
    \edge {t} {x};
    \edge {x} {t};
    \edge {t} {beta};
    \draw[->,blue] (x) to[out=45,in=135] (beta);
    
    \end{tikzpicture}\hfill
    \begin{tikzpicture}
    % Variables
    \node[const]   (t)   {$t$}; %
    \node[const, below=of t]   (xi)   {$\xi_t$}; %
    \node[const, below=of xi, xshift=-0.8cm]   (x)   {$x_t$}; %
    \node[const, below=of xi, xshift=0.8cm]   (beta)   {$\beta_t$}; %

    % Edges
    \edge {t} {xi};
    \edge {xi} {x};
    \edge {x} {xi};
    \edge {xi} {beta};
    \draw[->,blue] (x) to[out=45,in=135] (beta);
    
    \end{tikzpicture}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

==> tab/dietary_rmse.tex <==
\begin{table}[]
\centering
\caption{Dietary Weight Control Product Data --- RMSE Comparison}
\label{tab:dwc_rmse}
\begin{tabular}{cccc}
\hline
                   Nonlinear GP         & Dynamic GP           & Hill & Log Dynamic GP               \\ \hline
3.29             & 2.87             & 3.16 &    2.51         \\
 (2.18, 5.78)  & (1.82, 4.99) & (2.59, 4.69) & (1.47, 4.37) \\
 \hline
\end{tabular}
\end{table}

==> tab/nielsen_rmse.tex <==
\begin{table}[]
\centering
\caption{Nielsen Data --- RMSE Comparison}
\label{tab:nielsen_rmse}
\begin{tabular}{lcc}
\toprule
                   & Nonlinear (GP)         & Dynamic (GP)                        \\ \midrule
{Chocolate}  & 368,766             & 387,623                         \\
                   & (207,634, 601,163)  & (207,350, 671,246)  \\ \midrule
{Pet Food}  & 48,438              & 41,825                          \\
                   & (27,920, 83,249)   & (24,631, 65,232)      \\ \midrule
{Coffee}   & 722,076             & 733,269                         \\
                   & (509,527, 919,820) & (490,785, 994,303)  \\ \midrule
{Beer} & 443,817         &   423,085                                      \\ & (236,730, 911,732)
                   &    (207,914, 802,740)                                          \\ \bottomrule
\end{tabular}
\end{table}

==> xr.tex <==
\usepackage{xr}
\makeatletter

\newcommand*{\addFileDependency}[1]{% argument=file name and extension
\typeout{(#1)}% latexmk will find this if $recorder=0
% however, in that case, it will ignore #1 if it is a .aux or 
% .pdf file etc and it exists! If it doesn't exist, it will appear 
% in the list of dependents regardless)
%
% Write the following if you want it to appear in \listfiles 
% --- although not really necessary and latexmk doesn't use this
%
\@addtofilelist{#1}
%
% latexmk will find this message if #1 doesn't exist (yet)
\IfFileExists{#1}{}{\typeout{No file #1.}}
}\makeatother

\newcommand*{\myexternaldocument}[1]{%
\externaldocument{#1}%
\addFileDependency{#1.tex}%
\addFileDependency{#1.aux}%
}
%------------End of helper code--------------

% put all the external documents here!
%\myexternaldocument{web_appendix}
